Data-driven and Automatic Surface Texture Analysis Using Persistent Homology

Surface roughness plays an important role in analyzing engineering surfaces. It quantifies the surface topography and can be used to determine whether the resulting surface finish is acceptable or not. Nevertheless, while several existing tools and standards are available for computing surface roughness, these methods rely heavily on user input thus slowing down the analysis and increasing manufacturing costs. Therefore, fast and automatic determination of the roughness level is essential to avoid costs resulting from surfaces with unacceptable finish, and user-intensive analysis. In this study, we propose a Topological Data Analysis (TDA) based approach to classify the roughness level of synthetic surfaces using both their areal images and profiles. We utilize persistent homology from TDA to generate persistence diagrams that encapsulate information on the shape of the surface. We then obtain feature matrices for each surface or profile using Carlsson coordinates, persistence images, and template functions. We compare our results to two widely used methods in the literature: Fast Fourier Transform (FFT) and Gaussian filtering. The results show that our approach yields mean accuracies as high as 97%. We also show that, in contrast to existing surface analysis tools, our TDA-based approach is fully automatable and provides adaptive feature extraction.

==> sections/sec-surface_texture_simulation.tex <==
%!TEX root = ../ICMLA2019.tex
%*****************************
\section{Modeling}
\label{sec:milling_simulation}
%------------------------------------
We consider a milling operation with straight edge cutters as shown in Fig.~\ref{fig:up_down_milling}. 
A single degree of freedom model in the $x$ direction for the tool oscillations is used as shown in Fig.~\ref{fig:up_down_milling}a, and both upmilling and downmilling processes are considered in the analysis.  
The equation of motion that describes the tool oscillations is 
%------------------------------------
\begin {equation}
\label{eq:eom_end_mill}
\ddot{x}+ 2\zeta \omega_{n}\dot{x}+\omega_{n}^{2} x = \frac{1}{m} F(t),
\end{equation}
%------------------------------------
where $m$, $w_{n}$, $\zeta$ and $F(t)$ represent the modal mass, natural frequency, damping ratio and the cutting force in the $x$ direction, respectively. 
$\tau$ is the time delay given by $\tau = 2\pi/N\Omega$ where $\omega$ is the spindle's rotational speed in rad/s, while $N$ is the number of cutting edges or teeth. 
The expression for the cutting force is given by \cite{Altintas2009,Bobrenkov2010}
%-----------------------------------------
\begin{equation}
\label{eq:modified_cutting_force}
\begin{split}
F= \sum\limits_{n=1}^z \big[-bK_{t} g_n(t)( \cos{\theta_{n}(t)}+ \tan{\gamma} \sin{\theta_{n}(t)}) \sin{\theta_{n}(t)}\big]\\
\big[(f+x(t)-x(t-\tau))\big],
\end{split}
\end{equation}
%-----------------------------------------
where $\theta_{n}$ is the angle between the vertical line and the leading tooth of the cutting tool as shown in Fig.~\ref{fig:up_down_milling}. 
The constant $K_{t}$ is the linearized cutting coefficient in the tangential direction and $\tan{\gamma}=K_{n}/K_{t}$ where $K_n(t)$ is the cutting coefficient in the normal direction. 
The screening function $g_{n}(t)$ is either $0$ or $1$ depending on whether the $n$th tooth is engaged in the cut or not, respectively, and $f$ represents the feed per tooth of the cutting tool. 
The expression for angular position of the $n$th tooth $\theta_{n}(t)$ is given by \cite{Bobrenkov2010}
%-----------------------------------------
\begin{equation}
\theta_{n}(t) = (2\pi\Omega/60)t+2\pi(n-1)/z,
\end{equation}
%-----------------------------------------
where $z$ is the total number of cutting teeth while $\Omega$ is the rotational speed given in revolutions per minute (rpm).

%---------------
\begin{figure}[hbt!]
\centering
\includegraphics[width=0.40\textwidth,height=0.7\textheight,keepaspectratio]{milling_straight_cutter_up_and_down_mill}
\caption{Milling process illustrations. a) Upmilling b) Downmilling}
\label{fig:up_down_milling}
\end{figure}
%---------------

One of the important cutting parameters is the radial immersion ratio (RI) which is defined as the ratio of the radial depth of cut to the diameter of the cutting tool. 
Smaller radial immersions indicate shallower cuts and thus more intermittent contact between the tool and the workpiece, while higher radial immersions indicate deeper cuts with a more continuous contact.  
In our simulations for both downmilling and upmilling we set $RI=0.25$. 

Inserting Eq.~\eqref{eq:modified_cutting_force} into Eq.~\eqref{eq:eom_end_mill} results in
%--------------------------------------------------
\begin{multline}
\label{eq:modified_eom_milling}
\ddot{x}(t)+2\zeta \omega_{n}(t)\dot{x}(t)+w_{n}^{2}x(t)=\\
-\frac{bh(t)}{m}[x(t)-x(t-\tau)]-\frac{bf_{0}(t)}{m},
\end{multline}
%--------------------------------------------------
where $b$ is the nominal depth of cut and  $h(t)$ is the $\tau$-periodic function 
%--------------------------------------------------
\begin{multline}
h(t)=\sum\limits_{n=1}^z K_{t} g_n(t) \big[  \cos{\theta_{n}(t)}+\\ \tan{\gamma} \sin{\theta_{n}(t)} \big]  \sin{\theta_{n}(t)},
\end{multline}
%--------------------------------------------------
and $f_0(t)=h(t)\, f$. 
The term $f_0(t)$ does not affect the stability analysis, so we drop it in the subsequent equations; however we keep it in the simulation. 

After dropping $f_0(t)$, the equations of motion can be written in state space form according to
%--------------------------------------------------
\begin{equation}
\frac{d\boldsymbol{\xi}(t)}{dt} = \textbf{A}(t)\boldsymbol{\xi}(t)+\textbf{B}(t)\boldsymbol{\xi}(t-\tau),
\end{equation}
%--------------------------------------------------
where $\textbf{A}$ and $\textbf{B}$ are $T$-periodic with $T=\tau$. 
Then, using the spectral element method \cite{Khasawneh2011}, the state space is discretized and we obtain the dynamic map
%-----------------------------------------
\begin{equation}
\boldsymbol{\xi}_{n+1} = U\boldsymbol{\xi}_{n},
\end{equation}
%-----------------------------------------
where $\textbf{U}$ is the finite dimensional monodromy operator.  
The eignenvalues of $U$ approximate the eigenvalues of the infinite dimensional monodromy operator of the equation of motion. 
If the modulus of the largest eigenvalue is smaller than $1$, then the corresponding spindle speed and depth of cut pair leads to a chatter-free process; otherwise, chatter occurs. 
Therefore, the stability of the milling model and the bifurcation associated with the loss of stability (chatter) can be obtained by examining these eigenvalues, see Fig.~\ref{fig:stability_circle}. 

In this study, we generated $10000$ time series corresponding to a $100\times100$ grid in the plane of the spindle speeds and depths of cut. 
Each time series is tagged using the largest eigenvalue of the monodromy matrix corresponding to the same grid point. 

%---------------
\begin{figure}[hbt!]
\centering
\includegraphics[width=0.40\textwidth,height=0.7\textheight,keepaspectratio]{stabcirc}
\caption{Stability criteria used in this study based on the eigenvalues of the monodromy matrix $\textbf{U}$.}
\label{fig:stability_circle}
\end{figure}
%---------------
